BADGR: Bundle Adjustment Diffusion Conditioned by GRadients for Wide-Baseline Floor Plan Reconstruction

Reconstructing precise camera poses and floor plan layouts from wide-baseline RGB panoramas is a difficult and unsolved problem. We introduce BADGR, a novel diffusion model that jointly performs reconstruction and bundle adjustment (BA) to refine poses and layouts from a coarse state, using 1D floor boundary predictions from dozens of images of varying input densities. Unlike a guided diffusion model, BADGR is conditioned on dense per-entity outputs from a single-step Levenberg Marquardt (LM) optimizer and is trained to predict camera and wall positions while minimizing reprojection errors for view-consistency. The objective of layout generation from denoising diffusion process complements BA optimization by providing additional learned layout-structural constraints on top of the co-visible features across images. These constraints help BADGR to make plausible guesses on spatial relations which help constrain pose graph, such as wall adjacency, collinearity, and learn to mitigate errors from dense boundary observations with global contexts. BADGR trains exclusively on 2D floor plans, simplifying data acquisition, enabling robust augmentation, and supporting variety of input densities. Our experiments and analysis validate our method, which significantly outperforms the state-of-the-art pose and floor plan layout reconstruction with different input densities.

==> rebuttal/PuzzleFusion.tex <==
\begin{table}[h]
\centering
\vspace{-10pt}
\scalebox{0.8}{
% \begin{tabular}{ccccccccc}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}starting room poses, \\ imgs / rms\end{tabular}} & \multicolumn{4}{c}{Pose Err Dist} & \multicolumn{4}{c}{Visible Layout Err Dist} \\ \cline{2-9} 
%                                                                                             & Mn     & Med    & Std    & p90    & Mn       & Med       & Std       & p90      \\ \hline
% perfect, 1                                                                                  &        &        &        &        &          &           &           &          \\
% perfect, 2                                                                                  &        &        &        &        &          &           &           &          \\
% noisy, 1                                                                                    &        &        &        &        &          &           &           &          \\
% noisy, 2                                                                                    &        &        &        &        &          &           &           &          \\ \hline
% \end{tabular}

% \begin{tabular}{c|ccc}
% \hline
% Method  & \textit{E-SfM} & \textit{PF} & \textit{BADGR}  \\ \hline
% MPE(\%) & 11.5\%  & 3.4\%        & 0.33\% \\ \hline
% \end{tabular}

\begin{tabular}{llll}
\hline
MPE$\downarrow$ & E-SfM: 11.5\% & PF:3.4\% & BADGR:0.33\% \\ \hline
\end{tabular}
}
\vspace{-10pt}
\end{table}

==> rebuttal/graphcovis.tex <==
\begin{table}[ht]
\vspace{-10pt}
\centering
\scalebox{0.42}{
% \begin{tabular}{cc|cccccc|cccccc}
% \hline
% \multirow{2}{*}{\# Panos} & \multirow{2}{*}{Methods} & \multicolumn{3}{c}{Partially Rot (deg)} & \multicolumn{3}{c|}{Partially Dist (cm)} & \multicolumn{3}{c}{Fully Rot (deg)} & \multicolumn{3}{c}{Fully Dist (cm)} \\ \cline{3-14} 
%                           &                          & Mn          & Med         & Std         & Mn           & Med         & Std         & Mn         & Med       & Std        & Mn         & Med       & Std        \\ \hline
% \multirow{2}{*}{3}        & \textit{GC}                       & 5.36        & 1.36        & 15.92       & 34.0         & 12.4        & 99.3        & 1.86       & 0.83      & 8.71       & 6.9        & 3.7       & 20.8       \\
%                           & \textit{BG}                       & 0.25        & 0.20        & 0.28        & 9.9          & 7.0         & 4.2         &            &           &            &            &           &            \\ \hline
% \multirow{2}{*}{4}        & \textit{GC}                       & 9.01        & 1.40        & 25.24       & 38.6         & 13.7        & 81.1        & 1.75       & 0.87      & 7.40       & 9.5        & 5.2       & 22.6       \\
%                           & \textit{BG}                       & 0.26        & 0.22        & 0.30        & 10.2         & 8.2         & 4.5         &            &           &            &            &           &            \\ \hline
% \multirow{2}{*}{5}        & \textit{GC}                       & 4.71        & 1.32        & 13.57       & 24.6         & 12.6        & 46.2        & 2.43       & 0.95      & 10.92      & 12.8       & 6.4       & 31.9       \\
%                           & \textit{BG}                       & 0.25        & 0.19        & 0.30        & 9.3          & 7.7         & 4.7         &            &           &            &            &           &            \\ \hline
% \end{tabular}
\begin{tabular}{ccccccccccccc}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Group-Size\\ \# imgs\end{tabular}} & \multicolumn{3}{c}{GC Rot $\downarrow$ ($^\circ$)} & \multicolumn{3}{c}{BADGR Rot $\downarrow$ ($^\circ$)}           & \multicolumn{3}{c}{GC Transl. $\downarrow$ (cm)} & \multicolumn{3}{c}{BADGR Transl. $\downarrow$ (cm)}      \\ \cline{2-13} 
                            & Mn        & Med      & Std       & Mn            & Med           & Std           & Mn            & Med          & Std  & Dist (cm)     & Med          & Std          \\ \hline
3                           & 2.00      & 0.85     & 9.15      & \textbf{0.25} & \textbf{0.20} & \textbf{0.28} & \textbf{8.1}  & \textbf{3.8} & 29.2 & 9.2           & 6.1          & \textbf{5.9} \\
4                           & 3.19      & 0.94     & 13.36     & \textbf{0.26} & \textbf{0.22} & \textbf{0.30} & 15.3          & \textbf{6.1} & 43.0 & \textbf{10.6} & \textbf{6.1} & \textbf{6.0} \\
5                           & 3.29      & 1.07     & 12.04     & \textbf{0.25} & \textbf{0.19} & \textbf{0.30} & 17.2          & 8.2          & 38.4 & \textbf{10.4} & \textbf{6.3} & \textbf{6.7} \\ \hline
\end{tabular}
}
\vspace{-12pt}
\end{table}

==> rebuttal/roombreakdown.tex <==
\begin{table}[ht]
\vspace{-10pt}
\setlength{\tabcolsep}{2pt}
\centering
\scalebox{0.4}{
\begin{tabular}{cccc|cccc|cccc|cccc|cccc}
\hline
\multicolumn{4}{c|}{\# rooms per floor} & \multicolumn{4}{c|}{1 - 5}     & \multicolumn{4}{c|}{6 - 10}    & \multicolumn{4}{c|}{11 - 15}   & \multicolumn{4}{c}{\textgreater{}=16} \\ \hline
\# floors   & transl $\downarrow$   & rot $\downarrow$  & layout $\downarrow$  & 23.7\% & 11.5cm & 0.25$^\circ$ & 6.3cm & 44.5\% & 10.1cm & 0.23$^\circ$ & 6.1cm & 25.9\% & 10.3cm & 0.24$^\circ$ & 6.4cm & 5.9\%    & 11.3cm   & 0.40$^\circ$   & 8.6cm   \\ \hline
\end{tabular}
}
\vspace{-21pt}
\end{table}

==> sec/4_datasets.tex <==
\section{Datasets}
% \begin{itemize}
%     \item Zillow, redraw data and simulated camera poses
%     \Subitem{Not doing curved walls, islands, split floor}
%     \Subitem{Difference between redraw and final evaluation format}
%     \Subitem{Note that the final eval data is annotated, error exists meaning we will never get zero.}
%     \Subitem{Noise simulator during training.}
%     \item RPLAN and simulated camera poses
% \end{itemize}

==> tables/baseline.tex <==
\begin{table*}[htbp]
\centering
\caption{ Baseline approach.}
\scalebox{0.8}{
\begin{tabular}{|c|c|c|c|c|}
\hline
                      & Stage   & \#Img & Cluster & Code Available?                                                                                                        \\ \hline
Salve (2022)          & Coarse  & 2     & PGO     & \begin{tabular}[c]{@{}c@{}}Yes, but very hard to run. \\ Performance not as good as CovisPose\end{tabular}             \\ \hline
Graph-Covis (2023)    & Coarse  & 5     & MSP     & Yes                                                                                                                    \\ \hline
CovisPose (2022)      & Coarse  & 2     & MSP     & Yes                                                                                                                    \\ \hline
PanoPose (2024)       & Coarse  & 2     & MSP     & No                                                                                                                     \\ \hline
CovisPose+ PGO        & Coarse  & 2     & PGO     & Yes                                                                                                                    \\ \hline
Traditional SfM + BA? & Refined & n     & N/A     & \begin{tabular}[c]{@{}c@{}}Check again of new work same image modality. \\ Salve has reported this number\end{tabular} \\ \hline
\end{tabular}
}
\label{tab:baselines}
\end{table*}

==> tables/layout_errs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[H]
\vspace{3mm}
\caption{Layout Error}
\label{tab:zind_layout}
\centering
\scalebox{0.63}{
\begin{tabular}{ccccccccccc}
\hline
\multirow{2}{*}{Img/Rm} & \multirow{2}{*}{Method} & \multicolumn{4}{c}{Visible walls (cm)}                     & \multicolumn{4}{c}{Invisible walls (cm)} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\% Invis. \\ Walls\end{tabular}} \\ \cline{3-10}
                        &                         & Mn           & Med          & Std          & p90           & Mn        & Med     & Std     & p90      &                                                                             \\ \hline
\multirow{4}{*}{0.6}    & \textit{CovisPose}      & 14.0         & 8.0          & 12.8         & 32.4          & -         & -       & -       & -        & \multirow{4}{*}{50.8\%}                                                     \\
                        & \textit{CovisPose+}     & 11.5         & 6.9          & 10.5         & 26.0          & -         & -       & -       & -        &                                                                             \\
                        & \textit{BA-Only}        & 12.8         & 6.8          & 11.9         & 29.3          & -         & -       & -       & -        &                                                                             \\
                        & \textit{\textbf{BADGR}} & \textbf{7.1} & \textbf{4.5} & \textbf{6.7} & \textbf{15.3} & 11.2      & 6.1     & 7.1     & 21.2     &                                                                             \\ \hline
\multirow{4}{*}{1}      & \textit{CovisPose}      & 15.0         & 9.0          & 13.0         & 39.1          & -         & -       & -       & -        & \multirow{4}{*}{42.3\%}                                                     \\
                        & \textit{CovisPose+}     & 12.3         & 7.0          & 10.8         & 27.4          & -         & -       & -       & -        &                                                                             \\
                        & \textit{BA-Only}        & 12.6         & 6.7          & 11.4         & 27.5          & -         & -       & -       & -        &                                                                             \\
                        & \textit{\textbf{BADGR}} & \textbf{7.0} & \textbf{4.6} & \textbf{6.6} & \textbf{15.8} & 9.3       & 5.7     & 9.3     & 19.7     &                                                                             \\ \hline
\multirow{4}{*}{2}      & \textit{CovisPose}      & 14.7         & 8.8          & 12.5         & 33.6          & -         & -       & -       & -        & \multirow{4}{*}{38.1\%}                                                     \\
                        & \textit{CovisPose+}     & 12.0         & 7.0          & 9.0          & 26.0          & -         & -       & -       & -        &                                                                             \\
                        & \textit{BA-Only}        & 10.5         & 6.2          & 9.9          & 23.3          & -         & -       & -       & -        &                                                                             \\
                        & \textit{\textbf{BADGR}} & \textbf{6.4} & \textbf{4.4} & \textbf{5.9} & \textbf{13.9} & 8.8       & 5.4     & 8.7     & 18.9     &                                                                             \\ \hline
\multirow{4}{*}{3}      & \textit{CovisPose}      & 14.3         & 8.5          & 12.1         & 31.8          & -         & -       & -       & -        & \multirow{4}{*}{36.7\%}                                                     \\
                        & \textit{CovisPose+}     & 12.3         & 7.2          & 10.2         & 26.9          & -         & -       & -       & -        &                                                                             \\
                        & \textit{BA-Only}        & 10.6         & 6.2          & 9.0          & 22.1          & -         & -       & -       & -        &                                                                             \\
                        & \textit{\textbf{BADGR}} & \textbf{6.6} & \textbf{4.3} & \textbf{6.0} & \textbf{14.6} & 8.8       & 5.5     & 8.7     & 18.8     &                                                                             \\ \hline
\end{tabular}
}
\end{table}

==> tables/pose_errs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[H]
\vspace{5mm}
\caption{\footnotesize  Pose Error. \textit{CovisPose} is the original approach reported in \cite{nejatishahidin2023graph} to estimate global poses. We apply vanishing point snapping to pairwise poses prior to computing the global poses. This is \textit{CovisPose+} and used as the initialization approach for pose and walls. Note that \textit{BA}-Only and \textit{BADGR} only optimize camera poses and layouts. The rotation error is the same as \textit{CovisPose+}.}
\label{tab:zind_pose}
\scalebox{0.75}{
\begin{tabular}{ccccccccc}
\hline
                                                                     &                           & \multicolumn{3}{c}{Rotation($^\circ$)}                                                                             & \multicolumn{3}{c}{Translation(cm)}                                            &                                                                               \\ \cline{3-8}
\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Imgs/\\ Rm\end{tabular}} & \multirow{-2}{*}{Methods} & Mn                                   & Med                                  & Std                                  & Mn                       & Med                      & Std                      & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\#walls/ \\ \#panos\end{tabular}} \\ \hline
                                                                     & \textit{CovisPose}        & 1.83                                 & 1.25                                 & 1.48                                 & 22.9                     & 17.4                     & 13.4                     &                                                                               \\
                                                                     & \textit{CovisPose+}       & \textbf{0.24}                        & \textbf{0.20}                        & \textbf{0.30}                        & 20.7                     & 15.7                     & 12.0                     &                                                                               \\
                                                                     & BA Only                   & {\color[HTML]{9B9B9B} \textbf{0.24}} & {\color[HTML]{9B9B9B} \textbf{0.20}} & {\color[HTML]{9B9B9B} \textbf{0.30}} & 19.1                     & 12.2                     & 10.9                     &                                                                               \\
\multirow{-4}{*}{0.6}                                                & \textit{BADGR}            & {\color[HTML]{9B9B9B} \textbf{0.24}} & {\color[HTML]{9B9B9B} \textbf{0.20}} & {\color[HTML]{9B9B9B} \textbf{0.30}} & \textbf{12.2}            & \textbf{9.5}             & \textbf{7.2}             & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}59.4/\\ 8.0\end{tabular}}         \\ \hline
                                                                     & \textit{CovisPose}        & 1.88                                 & 1.36                                 & 1.40                                 & 23.0                     & 18.0                     & 13.2                     &                                                                               \\
                                                                     & \textit{CovisPose+}       & \textbf{0.26}                        & \textbf{0.21}                        & \textbf{0.30}                        & 19.7                     & 15.6                     & 11.8                     &                                                                               \\
                                                                     & BA Only                   & {\color[HTML]{9B9B9B} \textbf{0.26}} & {\color[HTML]{9B9B9B} \textbf{0.21}} & {\color[HTML]{9B9B9B} \textbf{0.30}} & \multicolumn{1}{l}{17.6} & \multicolumn{1}{l}{12.6} & \multicolumn{1}{l}{12.0} &                                                                               \\
\multirow{-4}{*}{1}                                                  & \textit{BADGR}            & {\color[HTML]{9B9B9B} \textbf{0.26}} & {\color[HTML]{9B9B9B} \textbf{0.21}} & {\color[HTML]{9B9B9B} \textbf{0.30}} & \textbf{11.2}            & \textbf{8.8}             & \textbf{6.5}             & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}65.7/\\ 10.4\end{tabular}}        \\ \hline
                                                                     & \textit{CovisPose}        & 1.90                                 & 1.49                                 & 1.31                                 & 22.3                     & 17.7                     & 12.6                     &                                                                               \\
                                                                     & \textit{CovisPose+}       & \textbf{0.26}                        & \textbf{0.19}                        & \textbf{0.30}                        & 17.9                     & 14.5                     & 10.2                     &                                                                               \\
                                                                     & BA Only                   & {\color[HTML]{9B9B9B} \textbf{0.26}} & {\color[HTML]{9B9B9B} \textbf{0.19}} & {\color[HTML]{9B9B9B} \textbf{0.30}} & \multicolumn{1}{l}{14.3} & \multicolumn{1}{l}{10.8} & \multicolumn{1}{l}{9.2} &                                                                               \\
\multirow{-4}{*}{2}                                                  & \textit{BADGR}            & {\color[HTML]{9B9B9B} \textbf{0.26}} & {\color[HTML]{9B9B9B} \textbf{0.19}} & {\color[HTML]{9B9B9B} \textbf{0.30}} & \textbf{10.7}            & \textbf{8.9}             & \textbf{6.0}             & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}65.9/\\ 16.0\end{tabular}}        \\ \hline
                                                                     & \textit{CovisPose}        & 1.70                                 & 1.19                                 & 1.23                                 & 21.5                     & 17.1                     & 11.9                     &                                                                               \\
                                                                     & \textit{CovisPose+}       & \textbf{0.23}                        & \textbf{0.19}                        & \textbf{0.27}                        & 18.1                     & 14.8                     & 10.5                     &                                                                               \\
                                                                     & BA Only                   & {\color[HTML]{9B9B9B} \textbf{0.23}} & {\color[HTML]{9B9B9B} \textbf{0.19}} & {\color[HTML]{9B9B9B} \textbf{0.27}} & \multicolumn{1}{l}{13.4} & \multicolumn{1}{l}{10.7} & \multicolumn{1}{l}{8.2} &                                                                               \\
\multirow{-4}{*}{3}                                                  & \textit{BADGR}            & {\color[HTML]{9B9B9B} \textbf{0.23}} & {\color[HTML]{9B9B9B} \textbf{0.19}} & {\color[HTML]{9B9B9B} \textbf{0.27}} & \textbf{10.6}            & \textbf{8.9}             & \textbf{6.0}             & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}66.5/\\ 18.3\end{tabular}}        \\ \hline
\end{tabular}
}
\vspace{-2mm}
\end{table}

==> tables/pose_errs_cliques.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[H]
\scalebox{0.75}{
\begin{tabular}{cccccccc}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Group\\ Size\end{tabular}} & \multirow{2}{*}{Methods} & \multicolumn{3}{c}{Rotation($^\circ$)} & \multicolumn{3}{c}{Translation(cm)} \\ \cline{3-8} 
                                                                      &                          & Mn          & Med         & Std        & Mn         & Med        & Std       \\ \hline
\multirow{3}{*}{Three}                                                & \textit{CovisPose}       &             &             &            &            &            &           \\
                                                                      & \textit{GraphCovis}      &             &             &            &            &            &           \\
                                                                      & \textit{BADGR}           & \textbf{}   & \textbf{}   & \textbf{}  & \textbf{}  & \textbf{}  & \textbf{} \\ \hline
\multirow{3}{*}{Four}                                                 & \textit{CovisPose}       &             &             &            &            &            &           \\
                                                                      & \textit{GraphCovis}      &             &             &            &            &            &           \\
                                                                      & \textit{BADGR}           &             &             &            & \textbf{}  & \textbf{}  & \textbf{} \\ \hline
\multirow{3}{*}{Five}                                                 & \textit{CovisPose}       &             &             &            &            &            &           \\
                                                                      & \textit{GraphCovis}      &             &             &            &            &            &           \\
                                                                      & \textit{BADGR}           &             &             &            &            &            &           \\ \hline
\end{tabular}
}
\end{table}

==> tables/room_shape_errs.tex <==
\begin{table}[H]
\centering
\vspace{3mm}
\caption{Single Room Layout Estimation}
\label{tab:layout_estim}
\scalebox{0.8}{
\begin{tabular}{cccccc}
\hline
Img/Rm               & Method           & Mn        & Med       & Std       & p90       \\ \hline
\multirow{3}{*}{1}   & \textit{LGT-Net} &           &           &           &           \\
                     & \textit{?-Net}   &           &           &           &           \\
                     & \textit{BADGR}   & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\ \hline
\multirow{3}{*}{2}   & \textit{LGT-Net} &           &           &           &           \\
                     & \textit{?-Net}   &           &           &           &           \\
                     & \textit{BADGR}   & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\ \hline
\multirow{3}{*}{All} & \textit{LGT-Net} &           &           &           &           \\
                     & \textit{?-Net}   &           &           &           &           \\
                     & \textit{BADGR}   &           &           &           &           \\ \hline
\end{tabular}
}
\end{table}

==> tables/rplan_noised_reproj.tex <==
\begin{table}[H]
\centering
\vspace{5mm}
\caption{Reprojection errors computed from on RPLAN dataset with simulated panorama poses and rendered floor boundaries.}
\scalebox{0.62}{
\begin{tabular}{cccccc}
\hline
\begin{tabular}[c]{@{}c@{}}Imgs/Rms\\ \%noise\end{tabular}                          & Method                  & Mn            & Med           & Std           & p90           \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}1\\ 5\% chance\\ 2\%scale\end{tabular}}  & \textit{CovisPose+}     & 12.69         & 7.54          & 16.56         & 28.7          \\
                                                                                    & \textit{BA-Only}        & 1.85          & \textbf{0.10} & 6.04          & 4.52          \\
                                                                                    & \textit{\textbf{BADGR}} & \textbf{0.84} & 0.22          & \textbf{3.23} & \textbf{1.37} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}1\\ 10\% chance\\ 2\%scale\end{tabular}} & \textit{CovisPose+}     & 12.88         & 7.33          & 17.03         & 29.06         \\
                                                                                    & \textit{BA-Only}        & 2.44          & \textbf{0.12} & 6.90          & 6.47          \\
                                                                                    & \textit{\textbf{BADGR}} & \textbf{1.10} & 0.24          & \textbf{3.76} & \textbf{1.77} \\ \hline
\end{tabular}
}
\label{tab:rplan_noised_reproj}
\end{table}

==> tables/rplan_reproj.tex <==
\begin{table}[H]
\centering
\vspace{5mm}
\caption{Reprojection errors computed from on RPLAN dataset with simulated panorama poses and rendered floor boundaries.}
\scalebox{0.62}{
\begin{tabular}{ccccccccc}
\hline
Img/Rm                  & \multicolumn{4}{c}{1}                                         & \multicolumn{4}{c}{2}                                         \\
Method                  & Mn            & Med           & Std           & p90           & Mn            & Med           & Std           & p90           \\ \hline
\textit{CovisPose+}     & 12.33         & 7.73          & 14.62         & 28.53         & 10.56         & 6.9           & 11.54         & 24.47         \\
\textit{BA-Only}        & 0.50          & \textbf{0.12} & 1.73          & 0.96          & 0.38          & \textbf{0.12} & 1.29          & 0.45          \\
\textit{\textbf{BADGR}} & \textbf{0.37} & 0.23          & \textbf{0.82} & \textbf{0.71} & \textbf{0.31} & 0.22          & \textbf{0.47} & \textbf{0.60} \\ \hline
\end{tabular}
}
\label{tab:rplan_reproj}
\end{table}
